To See or To Read: User Behavior Reasoning in Multimodal LLMs

Multimodal Large Language Models (MLLMs) are reshaping how modern agentic systems reason over sequential user-behavior data. However, whether textual or image representations of user behavior data are more effective for maximizing MLLM performance remains underexplored. We present \texttt{BehaviorLens}, a systematic benchmarking framework for assessing modality trade-offs in user-behavior reasoning across six MLLMs by representing transaction data as (1) a text paragraph, (2) a scatter plot, and (3) a flowchart. Using a real-world purchase-sequence dataset, we find that when data is represented as images, MLLMs next-purchase prediction accuracy is improved by 87.5% compared with an equivalent textual representation without any additional computational cost.

==> Sections/1-intro.tex <==
\section{Introduction}
\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/efficient_reasoning_fig1.pdf}
    \caption{A schematic showing different representations (text, scatter plot, and flow chart) of user history for next purchase prediction using multimodal LLMs.}
    \label{fig:motivation}
\end{figure}
%{\color{red}{Varun's to-do: add reference}}


The ability to reason about user behavior from sequential data is a cornerstone of modern intelligent systems, enabling applications such as personalized recommendation (transaction history), chatbot (dialogue history) and proactive user support (meeting notes) \citep{zhao2024recommender, singh2024historical}. Advancement in Multimodal Large Language Models (MLLMs) has fundamentally shifted the paradigm for this task, replacing specialized models with multimodal general-purpose reasoning engines \citep{li2024llms, shahriar2024putting}. 
% These models can process diverse customer behavior sequences—spanning e-commerce transactions, chatbot conversations, and social media history—to predict future intent and rationalize user actions. 
This new paradigm, however, introduces a critical and under-explored question: \textbf{how should sequential user histories be represented to optimize for both reasoning accuracy and computational efficiency} \citep{ai2024advancement, li2025graph, imam2025can, yang2025benchmarking}? This question is particularly critical in agentic recommendation systems \citep{huang2025towards, shang2025agentrecbench}, where understanding the user journey and their transition directly impacts personalization and revenue.

The complex user journey with a high-dimensional sequence of clicks, views, and purchases provides a representative testbed for this challenge via next purchase prediction \citep{chen2022sequential}. Effective reasoning requires capturing latent intent and its transition from these sequences, such as distinguishing ``goal-oriented price comparison" from ``aimless browsing" \citep{bauboniene2015commerce, zeng2020user}. The standard approach of feeding MLLMs a flattened, line-by-line textual transcript of these events preserves granular detail, but it losses the structural information of user journey such as topological pattern. Consequently, this method can be inefficient and fail to grasp the holistic user narrative, degrading the quality of intent prediction.

To address this question, we introduce \texttt{BehaviorLens}, a systematic benchmarking framework for evaluating modality trade-offs in user behavior reasoning. \texttt{BehaviorLens} directly compares two representations for the same user history: (i) a high-fidelity textual transcript and (ii) a holistic visual rendering. We evaluate these using state-of-the-art MLLMs on a next-purchase prediction task with a fixed candidate set, assessing both the prediction and the computational cost. Applied to real-world user transaction data, \texttt{BehaviorLens} reveals a key finding: holistic image representations of user history can help improve next-purchase prediction accuracy when compared to text representations, with no additional computational cost.

By systematically comparing modalities under controlled conditions, \texttt{BehaviorLens} contributes both a reproducible methodology for evaluating multimodal reasoning and empirical insights into the efficiency-performance trade-offs of input representations. Beyond next purchase prediction, our framework provides a template for optimizing user historical data streams for MLLMs in any domain involving complex sequential data, supporting future research on efficient context management, data compression, and the development of more robust reasoning systems.

% To address this question, we conduct a systematic investigation by revisiting these claims in the context of next purchase prediction from user histories, a classic task in personalization and recommender systems. Unlike prior work, we directly compare textual sequential encodings with image encodings of the same user histories, using the same MLLM and the same multiple-choice candidate set. The LLM is asked to (1) predict the next purchased product type and (2) provide reasoning for its decision. The empirical experiment results show that, contrary to prior claims, visual compression may not aid LLM reasoning for fine-grained categorical prediction tasks. 

% Our primary contribution is a principled analysis of the modality trade-off for multimodal user reasoning, providing a clear answer to the "to see or to read" dilemma. Our findings reveal that visual representations can achieve comparable or superior reasoning performance at a fraction of the computational cost for high-level planning tasks, while textual inputs maintain an edge for fine-grained, detail-oriented predictions. This work directly contributes to the core topic of the efficient reasoning workshop by demonstrating that input representation is a critical, yet often overlooked, lever for optimizing the computational efficiency of LLM-based reasoning systems. By understanding these trade-offs, practitioners can make more informed design choices for building scalable and cost-effective user behavior modeling systems.

% Large Language Models (LLMs) are increasingly used for reasoning over structured sequences, from natural language to event logs. Recent researches argue that compressing sequential data into visual representations, such as knowledge graphs, flow charts, or heatmaps can make LLM reasoning more efficient. For example, \citet{ai2024advancement} reports that compared to graph neural models or heuristic graph-to-text instruction, image encoding by Vision-Language Models (VLMs) can facilitate LLM-based reasoning over structured data. Similarly, the work of \citet{li2025graph} shows that visual representations aid multi-graph reasoning tasks.


% In this paper, we revisit these claims in the context of next-item prediction from customer purchase histories, a task in e-commerce personalization and recommender systems. Unlike prior work, we directly compare textual sequential encodings with image encodings of the same customer histories, using the same LLM and the same multiple-choice candidate set. The LLM is asked to (1) predict the next purchased product type and (2) provide reasoning for its decision. The empirical experiment results show that, contrary to prior claims, visual compression may not aid LLM reasoning for fine-grained categorical prediction tasks. 



==> Sections/2-related_works.tex <==
\section{Related Works}
%{\color{red}{Varun's to-do: add reference if any}}

\subsection{Next Item Prediction}
Classical approaches to next item prediction include Markov chains, matrix factorization, and factorization machines, which model user–item interactions using latent factors. With the rise of deep learning, recurrent neural networks such as GRU4Rec \citep{hidasi2016sessionbasedrecommendationsrecurrentneural} became influential in modeling sequential recommendation, capturing order-dependent behaviors in clickstreams and purchase sequences. Transformer-based architectures, such as SASRec \citep{kang2018selfattentivesequentialrecommendation} and BERT4Rec \citep{sun2019bert4recsequentialrecommendationbidirectional}, further advanced next-item prediction by leveraging self-attention to model long-range dependencies in user behavior.

Beyond sequential modeling, graph-based approaches such as SR-GNN \citep{10.1609/aaai.v33i01.3301346} and GCE-GNN \citep{10.1145/3397271.3401142} introduced graph neural networks for capturing complex item–item relations in session-based recommendation. Other notable advances include Caser \citep{10.1145/3159652.3159656}, which treats user-item interactions as sequences of images, and STAMP \citep{10.1145/3219819.3219950}, which focuses on capturing users’ short-term interests for better next-item prediction.

Despite significant improvements in accuracy, these models have limited interpretability of why a particular item is predicted. This has led to a growing interest in approaches that not only predict but also explain user preferences, paving the way for the integration of large language models into recommendation tasks.

\subsection{LLM for Recommendation and Reasoning}
Large language models (LLMs) such as GPT, LLaMA, and PaLM have recently been explored for recommender systems by framing user histories and items as natural language. Early explorations such as LLMRec \citep{10.1145/3616855.3635853} and ReXPlug \citep{10.1145/3404835.3462939} showed that LLMs can adapt to recommendation tasks with minimal fine-tuning, leveraging their world knowledge to infer user preferences. Other works like P5 proposed a unified framework that casts different recommendation problems into text-to-text tasks, demonstrating the flexibility of LLMs as general-purpose recommenders.

One of the distinctive advantages of LLMs is their ability to generate reasoning alongside predictions. Models such as ChatRec and Explainable GPT-based Recommenders show that natural language explanations can improve user trust and system transparency. Despite these advances, most existing work evaluates LLM reasoning in text-only settings \citep{gao2023chat}. Little is known about how LLMs reason when user histories are compressed into images. Our work is among the first to directly compare the reasoning efficiency of LLMs across textual and image-based representations of customer journeys, expanding the discussion from prediction accuracy to reasoning quality.

\subsection{Multi-Modal Representations of Customer Journey}
Beyond text-based sequence modeling, more work explores the idea of transforming sequential user interactions into image-like representations that can be processed by convolutional or vision-inspired models. For example, Markov Transition Fields (MTF) and Gramian Angular Fields (GAF) transform time series into images, enabling CNNs to extract spatial dependencies that are otherwise hard to capture in sequential models. In the recommender systems domain, Caser explicitly modeled sequential user–item interactions as a 2D ``image” where convolutional filters capture local sequential patterns as well as high-level transition features. Similarly, DeepMove leveraged trajectory data by representing spatio-temporal patterns in image-like forms to predict next locations, which parallels the idea of encoding customer journeys for next-item prediction \citep{zhou2018deepmove}. 

More recent work has used self-attention and visual encodings to compress large-scale sequential behaviors into compact 2D structures. For instance, Time2Graph converts multivariate sequences into graph-like images \citep{cheng2020time2graph}, while Rec2Image proposed encoding user behavior sessions into image matrices, enabling CNNs to identify higher-order dependencies. These studies demonstrate that compressing sequential histories into visual representations not only reduces input complexity but also allows reasoning models to leverage spatial proximity and clustering cues that may be less salient in raw text sequences. 

Despite these advances, prior work primarily used CNN-based architectures for learning from compressed images. Little is known about how large language models (LLMs) reason when fed such image-based summaries compared to traditional text sequences. Our work extends this line of research by investigating reasoning efficiency in LLMs when user journeys are compressed into scatter plot–like images, directly comparing prediction performance and the quality of generated reasoning across modalities.

==> Sections/3-method.tex <==
\section{Methodology}   
An agentic recommendation system relies on MLLM's reasoning of user history to understand the user intent. Formally, the reasoning process could be defined as an optimization of the recommendation policy $\pi(a)$ given the user $u$'s history,
\begin{equation}
    \text{max}_{\pi(a)} \mathbb{E} [\mathcal{R}_{MLLM}(u, [\phi(a, i, e)]_n)) | \pi(a)],
\end{equation}
where $\mathcal{R}$ refers to the utility score of user reasoning based on the last $n$ interactions $[\phi(a, i, e)]_n$. Each interaction is defined by a set of actions $a \in A$ (e.g., purchase), a set of engaged items $i \in \mathcal{I}$, and the environment context $e \in \mathcal{E}$ (e.g., timestamp).
We study the impact of user behavior representation function $\phi(a, i, e)$ on user intent reasoning efficiency $\mathcal{R}$.

\subsection{User Behavior Representations}
We compare three ways of representing the user journey as MLLM input with the focus on the purchase history, $a = \text{``purchase''}$.  

\noindent \textbf{Textual Sequential Representation}: the widely-adopted solution for user modeling \citep{liao2023llara} where each tuple $(a, i, e)$ is represented as a natural language description 
\begin{equation}
    \phi_{text}(a, i, e) = \text{``\textit{item \{i\} was \{a\} at timestamp \{e\}}''},
\end{equation}
and the purchase history $[\phi(a, i, e)]_n$ is a concatenation of all the purchase event description.  


\noindent \textbf{Scatter-plot Representation}: The same purchase history is transformed into a scatter plot image to visualize the temporal patterns as a time series. It is inspired by visualization in time-series modeling tasks \citep{wang2015image}, 
\begin{equation}
    \phi_{scatter-plot}(a, i, e) = \text{plot}(a, i | x = r(e), y=r(i)).
\end{equation}
Here, $r(\cdot)$ denotes a transformation function to map the value into the coordinate system. For example, $r(\cdot)$ could be a ranking function, mapping each input element to its corresponding ordinal rank. 

\noindent \textbf{Flow-chart Representation}: Inspired by recent work that claims visual compression aids LLM reasoning in structured tasks \citep{li2025graph}, the same purchase history is transformed into a flowchart where purchases as nodes are connected to keep temporal proximity. Typically, we recursively define the flowchart conversion as
\begin{equation}
    \phi_{flowchart}(a, i, e) = \text{node}(a, i, e | p=\{\text{node}(a_{-1}, i_{-1}, e_{-1})\}, s=\{\text{node}(a_{+1}, i_{+1}, e_{+1})\}),
\end{equation}
where the predecessor node set $p$ and the successor node set $s$ only contains the interaction ranked chronologically before ($e_{-1})$ and after ($e_{+1}$) the current interaction $(a, i, e)$, respectively.

\subsection{User Intent Prediction and Reasoning}
For each user, an MLLM receives either the text or the image representation, and is asked to: (1) predict the most likely next purchase $\pi(a)$ from a recall set, (2) provide explanation for the prediction. 
%The model outputs are compared against the ground-truth ``next product purchased" by the user. 
For each representation, we compare the prediction $\pi(a)$ with the ground-truth user behavior, measure the computational cost using token count as a proxy, and evaluate the generated explanation using LLM-as-a-Judge. 

==> Sections/4-experiments.tex <==
\section{Experiments}
% This section identifies which representation offers the best balance between accuracy and efficiency by comparing results and reasoning by different encodings across several advanced MLLMs. To evaluate performance in next-item prediction, we define the prediction accuracy as the percentage of exact matched predictions with ground truth, and define the similarity score as the average of cosine similarities between predictions and ground truth. To further illustrate reasoning efficiency, we consider metrics as causality, overthinking score, faithfulness, sufficiency, specificity, and plausibility.
% Additional details on our experimental setup, evaluation criteria, and prompt design are provided in the Appendix.

%% Examples, feel free to uncomment the first paragraph and make your changes. But the idea is to be very focused on the insight sharing. Think about making a post in 4-page, and leave details in appendix when people ask, only show essential definition. 

In this section we summarize which representation offers the best balance between reasoning accuracy and computational efficiency. See \autoref{sec:dataset_and_metrics} for details on the dataset and the experimental setup and \autoref{sec:prompts-reasoning} for the full prompts used in the experiments. 


%\begin{wraptable}{r}{0.8\textwidth}
\begin{table}[!h]
\centering
\caption{Comparison of MLLM reasoning performance with text vs image inputs.}
\begin{tabular}{lccccc}
\toprule
LLM Model & Input Type &  Accuracy  &  Similarity & Token Count & Latency(second)\\
\midrule
 Gemini-2.0-flash-lite & Text & 0.260 & 0.500 & 1233.46 & 1.510\\
Gemini-2.0-flash-lite & Scatterplot & \textbf{0.270} & \textbf{0.528} & 3560.49 & 2.338\\
 Gemini-2.0-flash-lite & Flowchart  & 0.260 & 0.517 & 1525.07 & 1.993\\
\midrule 
 Gemini-2.0-flash & Text & 0.240 & 0.483 & 1228.85 & 1.444\\
 Gemini-2.0-flash & Scatterplot & 0.270 & 0.510 & 3596.50 & 4.580\\
 Gemini-2.0-flash & Flowchart & \textbf{0.310} & \textbf{0.526} & 1529.35 & 4.977\\
\midrule 
 Gemini-2.5-flash-lite & Text & 0.360 & 0.570 & 1219.72 & 1.444\\
 Gemini-2.5-flash-lite & Scatterplot & \textbf{0.530} & \textbf{0.689} & 3623.25 & 2.057\\
 Gemini-2.5-flash-lite & Flowchart & 0.300 & 0.530 & 1566.41 & 1.814\\
\midrule 
 Gemini-2.5-flash & Text & \textbf{0.260} & \textbf{0.479} & 3585.01 & 1.444\\
 Gemini-2.5-flash & Scatterplot & 0.210 & 0.471 & 7223.44 & 6.003\\
 Gemini-2.5-flash & Flowchart & 0.220 & 0.447 & 5281.78 & 4.966\\
\midrule 
% Gemini-2.5-pro & Text & 0.270 & 0.524 \\
% Gemini-2.5-pro & Scatterplot \\
% Gemini-2.5-pro & Flowchart \\

 GPT-4o & Text & 0.420 & 0.602 & 1105.52 & 5.451\\
 GPT-4o & Scatterplot & \textbf{0.560} & \textbf{0.713} & 1169.48 & 8.954\\
 GPT-4o & Flowchart & 0.300 & 0.527 & 1042.78 & 7.140\\
\midrule 
 GPT-4.1-mini & Text & 0.320 & 0.542 & 1105.27 & 4.680\\
 GPT-4.1-mini & Scatterplot & \textbf{0.600} & \textbf{0.726} & 1039.24 & 7.849\\
 GPT-4.1-mini & Flowchart & 0.340 & 0.563 & 862.07 & 6.051\\

% GPT-o1 & Text & 0.250 & 0.491 \\
% GPT-o1 & Scatterplot  \\
% GPT-o1 & Flowchart \\

\bottomrule
\end{tabular}
 \label{tab:llm_reasoning_metrics}
\end{table}
%\end{wraptable}

\subsection{Results}
% \subsection{Evaluation Results}
Table \ref{tab:llm_reasoning_metrics} shows that representing customer journeys as images helps improve the accuracy, and the similarity score (i.e. cosine similarity of prediction and ground truth in text embeddings). With all the MLLMs, except Gemini-2.5-flash, either scatterplot or flowchart representation results in better prediction than the text representation. Image input achieves at most 33.9\% improvement in similarity score and 87.5\% improvement in prediction accuracy. This improvement is observed in both larger models, such as GPT-4o, and smaller models, such as GPT-4.1-mini and Gemini-2.5-flash-lite \citep{hurst2024gpt, comanici2025gemini}. The structure of image representations could further make a significant difference in accuracy. For flowchart, it shows better accuracy and similarity especially for Gemini-2.0-flash and Gemini-2.5-flash, while other MLLMs prefer scatterplot.

Table \ref{tab:llm_reasoning_metrics} also shows the computational cost in terms of the total number of tokens used by each MLLM. In Gemini models, flowchart and text input have similar token usage while scatter plots require more tokens. In GPT models, token usage remains at the same level for different representations, while accuracy is significantly higher for image representations. Table \ref{tab:llm_reasoning_metrics} further illustrates the latency as the request time in seconds for each MLLM for reference.

%Image reasoning was shorter with 58 tokens and less redundant with 19.5\% of average redundancy rate, but included more irrelevant mentions as overthinking density to be 0.97, and less efficient as accuracy per token to also favor text reasoning. Our evaluation results show while image reasoning is more concise and less redundant, it sacrifices prediction accuracy and introduces more irrelevant exploration. In contrast, textual representations of sequential histories maintain stronger alignment with the ground truth, providing more efficient reasoning per word. This contrasts with recent work that reported benefits of visual sequence compression for reasoning tasks, highlighting that fine-grained categorical prediction in consumer behavior may require textual sequence fidelity rather than image compression.




%emphasis it's different from prediction accuracy
% {\color{red} To illustrate if it is the input structure leading to improvement in the user behavior reasoning or if other parts of MLLMs also affect the prediction accuracy, we further deep dive into the explanations given by MLLMs.} 
To better understand whether the improvement in next purchase prediction is impacted by input representations or also impacted by intermediate explanations provided by MLLMs based on understanding of input, we define six metrics to evaluate the quality of explanations. The metrics are faithfulness, overthinking score, causality, sufficiency, specificity, and plausibility. We use LLM-as-a-judge for the evaluation \citep{gu2025surveyllmasajudge}. Prompts used by the judge are provided in \autoref{sec:prompts-eval}. Results are summarized in Figure \ref{fig:reasoning}, which show that the quality of explanations on understanding input representations is not significantly different across different inputs, except Gemini-2.0-flash model. This suggests that the choice of user history representation is the primary driver of improvement in next purchase prediction.


%different representations of user journey are the key factor to enhance user behavior reasoning by MLLMs.

%To better understand the impact of input representations on user behavior reasoning, we define six metrics to evaluate the quality of intermediate explanations provided by the model. The metrics are faithfulness, overthinking score, causality, sufficiency, specificity, and plausibility. We use LLM-as-a-judge for the evaluation \citep{gu2025surveyllmasajudge}. Results are summarized in Figure \ref{fig:reasoning}, which show that the quality metrics are not significantly different across different inputs, except Gemini-2.0-flash model. This proves that the different representations of user journey are the key factor to enhance user behavior reasoning by MLLMs.

% or if other parts of MLLMs also affect the prediction accuracy, we further deep dive into the explanations given by MLLMs.

% To better understand whether the improved prediction accuracy with visual representations stems from enhanced user behavior reasoning, we further analyze the explanations generated by each model. 

% To do this, we define six reasoning quality metrics: faithfulness, overthinking score, causality, sufficiency, specificity, and plausibility, and ask an LLM to evaluate the reasoning output by each model \citep{gu2025surveyllmasajudge}. Results are summarized in Figure \ref{fig:reasoning}, which show that the reasoning metrics are not significantly different across different inputs, except Gemini-2.0-flash model. These results suggest that improvements in prediction accuracy with visual representations may not be fully captured by these reasoning metrics. This points to a potential disconnect between surface-level reasoning quality and the underlying reasoning processes within MLLMs. In other words, while visual representations help the model make better predictions, the explanations it provides do not necessarily reflect that improvement. 





%We define 6 dimensional metrics as faithfulness, overthinking score, causality, sufficiency, specificity, and plausibility, and ask an LLM to evaluate the output reasoning for each MLLM \citep{gu2025surveyllmasajudge}.} Results are summarized in Figure \ref{fig:reasoning}. The metrics are not significantly different for different inputs except Gemini-2.0-flash. Note that these 6 metrics for reasoning evaluation are defined from a different perspective, compared to accuracy and similarity in order to measure predictive power of user behavior reasoning. {\color{red} This indicates reasoning grounding to the truth and with good rationality does not necessarily lead to good enough prediction results.}

%For example, in Gemini-2.0-flash, as for prediction accuracy and similarity, flowchart is better than scatterplot while text input has lowest prediction accuracy. Meanwhile, for reasoning by Gemini-2.0-flash, text input is better than flowchart or scatterplot, except for overthinking scores. 

%{\color{red}{Varun's to-do: help check result and conclusion}}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/llm_reasoning.png}
    \caption{Comparison in MMLM explanations. Each metric is measured by a scale of 1 to 5. Higher score indicates better reasoning in given metric. Blue dots are reasoning of text input. Green dots are reasoning of scatterplot input. Red dots are reasoning of flowchart input.}
    \label{fig:reasoning}
\end{figure}

%\lipsum[1-2]

\subsection{Case Study}
Given the sample user prompts in \autoref{sec:prompts-reasoning}, take the output from Gemini-2.5-flash as an example to understand difference in reasoning and prediction for different inputs. The sample customer actually purchased items from Crackers and Granola Bars after the most recent 20 purchases provided as input. 

In the reasoning by text input, it focuses more on the frequency of purchase patterns to predict next item as Cola, while also mentions different possibilities as snacks, which are close to user's next choice in reality. In the reasoning by flowchart input, it focuses more on the recency of purchase and considers the complementary item for the last purchased item. In the reasoning of scatterplot input, it better captures the recurring pattern of purchase, which is unique compared to the other two inputs, and leads to the correct prediction matching with user's interest.

\begin{promptbox}{Output from Text Input}
\textbf{PREDICTION:}
Cola.

\textbf{REASONING:}
The customer purchased Coca-Cola Classic Soda Pop Fridge Pack on both 2019-10-26 and 2019-11-01. This demonstrates a consistent and recurring need for this specific product type, making it highly probable for a subsequent purchase. While other options like Pastries (given the purchase of Toaster Pastries) or other snack/breakfast items are plausible, the direct repeat purchase of Cola makes it the strongest prediction.
\end{promptbox}


\begin{promptbox}{Output from Flowchart Input}
\textbf{PREDICTION:}
Pastries.

\textbf{REASONING:}
The last recorded purchase (indicated by arrow 19) was 100\% Arabica Medium Roast Ground Coffee Pods. Coffee is frequently consumed with breakfast items or snacks. Looking at the user's past purchases, they have previously bought Frosted Toaster Pastries (transaction 14), which falls under the Toaster Pastries product type. This indicates a preference for pastry-like items. Therefore, Pastries is a highly probable next purchase as it complements coffee and aligns with the user's established buying habits for breakfast/snack items.
\end{promptbox}

\begin{promptbox}{Output from Scatterplot Input}
\textbf{PREDICTION:}
Granola Bars.

\textbf{REASONING:}
The user's purchase history shows a recurring pattern of buying Multi Pack Snacks. The most recent purchase (order 20) was Classic Potato Chips, which falls under the Multi Pack Snacks category. Prior to that, OREO Cookie Sticks 'N Creme Dip Snack Packs (order 12) was also purchased from this category. Granola Bars are a very common and popular type of snack item, often sold in multi-packs, making them a highly plausible next purchase to replenish or vary the user's snack supply, directly continuing a recent and established purchasing trend.
\end{promptbox}


\par\vspace{\baselineskip}


==> Sections/5-conclusion.tex <==
\section{Conclusion}
% In this paper, we discuss the efficiency of user behavior reasoning with different encodings of user purchase log, and observe significant improvement in prediction accuracy with image representation. This finding enhances understanding of the user journey in MLLMs and further benefits personalization in agentic recommendation systems.
% In the future work, more exploration can focus on further optimizing image representation of user journey so that the temporal and spatio information can be better structured. 

In this paper we investigate the efficiency of reasoning over sequential user behavior data using different representations. We observe significant improvement in prediction accuracy with image representations. This finding advances our understanding of how MLLMs interpret the user journey and holds promise for enhancing personalization in agentic recommendation systems. Future work can focus on further optimizing the visual representations of the user journey to better capture temporal and spatial dynamics in the behavior. Future work should also investigate the impact of longer customer behavior sequences and should benchmark the study on a larger dataset.

%perspectives of reasoning evaluation besides prediction quality and rationality, which could help better understand root cause of how image representations are incorporated in user behavior reasoning.
